Learning for Single-Shot Confidence Calibration in Deep Neural Networks through Stochastic Inferences

We propose a generic framework to calibrate accuracy and confidence of a prediction in deep neural networks through stochastic inferences. We interpret stochastic regularization using a Bayesian model, and analyze the relation between predictive uncertainty of networks and variance of the prediction scores obtained by stochastic inferences for a single example. Our empirical study shows that the accuracy and the score of a prediction are highly correlated with the variance of multiple stochastic inferences given by stochastic depth or dropout. Motivated by this observation, we design a novel variance-weighted confidence-integrated loss function that is composed of two cross-entropy loss terms with respect to ground-truth and uniform distribution, which are balanced by variance of stochastic prediction scores. The proposed loss function enables us to learn deep neural networks that predict confidence calibrated scores using a single inference. Our algorithm presents outstanding confidence calibration performance and improves classification accuracy when combined with two popular stochastic regularization techniques---stochastic depth and dropout---in multiple models and datasets; it alleviates overconfidence issue in deep neural networks significantly by training networks to achieve prediction accuracy proportional to confidence of prediction.

==> sections/derivations.tex <==
% !TEX root = ../cvpr2019_conference.tex

\section{Stochastic depth as approximate Bayesian inference}

Residual networks (ResNets) \cite{he2016deep} propose to add skip connections to the network. Let $x_i$ denotes the output of the $i^{th}$ layer and $f_i(x)$ is commonly defined a typical convolutional transform from layer $i-1$ to $i$, then we obtain
\begin {align}
	\x_i = f_i(\x_{i-1}) + \x_{i-1}
\end {align}
and $f_i(x)$ is commonly defined by
\begin {align}
	f_i(\x) = W_i \cdot \sigma(B({W_i}' \cdot \sigma(B(\x))))
\end {align}
where $W_i$ and ${W_i}'$ are weight matrices, ($\cdot$) denotes convolution, and $B$ and $\sigma$ indicates batch normalization and ReLU function, respectively.

Let $e_i \in \{0, 1\}$ denotes a Bernoulli random variable which indicates whether the $i^{th}$ residual block is active or not, then we can represent ResNet with stochastic depth \cite{huang2016deep} as
\begin {align}
	\x_i = e_i f_i(\x_{i-1}) + \x_{i-1}
\end {align}
Then we can transform stochasticity from layers to the parameter space as follows:
\begin {align}
	f_i (\x_{i-1}) &= W_i \cdot \sigma(B({W_i}' \cdot \sigma(B'(\x_{i-1})))) \\
	e_i f_i (\x_{i-1}) + \x_{i-1} &= e_i \big ( W_i \cdot \sigma(B({W_i}' \cdot \sigma(B'(\x_{i-1})))) \big)+ \x_{i-1} \\
	&= e_i^4 \big ( W_i \cdot \sigma(B({W_i}' \cdot \sigma(B'(\x_{i-1})))) \big)+ \x_{i-1} \\
	&= e_i^4 \bigg (W_i \cdot \sigma(\gamma_i({{{W_i}' \cdot \sigma(B'(\x_{i-1}))-\mu_i}\over{\delta_i}})+\beta_i ) \bigg)+ \x_{i-1} \\
	&= e_i W_i \cdot \sigma(
	e_i \begin{bmatrix}
	\gamma_i \\ \beta_i
	\end{bmatrix}^T
	\begin{bmatrix}
	{1\over{\delta_i}}({{{e_i W_i}' \cdot \sigma(e_i \gamma_i'(\overline{\x_{i-1}}+\beta_i'))-e_i \mu_i}}) \\ 1  
	\end{bmatrix} ) + \x_{i-1}\\
	&= \widetilde{W_i} \cdot \sigma(
	\begin{bmatrix}
	\widetilde{\gamma_i} \\ \widetilde{\beta_i}
	\end{bmatrix}^T
	\begin{bmatrix}
	{1\over{\delta_i}}({{{\widetilde{W_i}}' \cdot \sigma(\widetilde{\gamma_i'}(\overline{\x_{i-1}}+\widetilde{\beta_i'}))-e_i \mu_i}}) \\ 1  
	\end{bmatrix} ) + \x_{i-1}\\
	&= f_{\widetilde{W_i}, \widetilde{W_i}', \widetilde{\gamma_i}, \widetilde{\gamma_i}', \widetilde{\beta_i}, \widetilde{\beta_i}' } (\x_{i-1}) = f_{\widetilde{\omega_i}} (\x_{i-1})
\end {align} 
$e_i = e_i^4$ since it is a Bernoulli random variable. All stochastic parameters ${\widetilde{\omega}_i} = {[\widetilde{W_i}, \widetilde{W_i}', \widetilde{\gamma_i}, \widetilde{\gamma_i}', \widetilde{\beta_i}, \widetilde{\beta_i}' ]}$ in this block drop at once or not.


\section{Proof of KL Condition}

Let  $\omega \in \mathbb{R}^D$, $p(\omega) = \mathcal{N}(0,\mathbf{I})$ and $q_\theta(\omega) = \sum_{i=1}^2 e_i \mathcal{N}(\theta_i, \sigma^2\mathbf{I})$ with a probability vector $\mathbf{e} = (e_1, e_2)$ where $e_i \in [0, 1]$. In our work, $\theta_1$ denotes the deterministic model parameter $[{W_i}, {W_i}', {\gamma_i}, {\gamma_i}', {\beta_i}, {\beta_i}' ]$ and $\theta_2=0$.
\begin{align}
\mathrm{KL}(q_\theta(\omega) || p(\omega)) &= \int q_\theta(\omega) \log \frac{q_\theta(\omega)}{p(\omega)}  d\omega \\
&= \int q_\theta(\omega) \log q_\theta(\omega)d\omega - \int q_\theta(\omega) \log p(\omega)  d\omega
\end{align}
We can re-parameterize the first entropy term
\begin{align}
\int q_\theta(\omega) \log q_\theta(\omega)d\omega &= \sum_{i=1}^2 e_i \int \mathcal{N}(\omega; \theta_i, \sigma^2_i\mathbf{I}) \log q_\theta(\omega) d\omega
\end{align}
by using $\omega = \theta_i + \sigma \epsilon_i$ with $\epsilon_i \sim \mathcal{N}(0,\mathbf{I})$, then
\begin{align}
\int q_\theta(\omega) \log q_\theta(\omega)d\omega &= \sum_{i=1}^2 e_i \int \mathcal{N}(\epsilon_i; 0, \mathbf{I}) \log q_\theta(\theta_i+ \sigma \epsilon_i) d\omega
\end{align}

Using $q_\theta(\theta_i+ \sigma \epsilon_i) \approx e_i (2 \pi)^{-D/2} \sigma^{-1} \exp ( -\frac{1}{2} \epsilon_i^{T} \epsilon_i )$ for large enough $D$,

\begin{align}
\int q_\theta(\omega) \log q_\theta(\omega)d\omega &= \sum_{i=1}^2 e_i \int \mathcal{N}(\epsilon_i; 0, \mathbf{I}) \log\big(e_i (2 \pi)^{-D/2} \sigma^{-1} \exp ( -\frac{1}{2} \epsilon_i^{T} \epsilon_i )\big) d\omega \\
&= \sum_{i=1}^2 \frac{e_i}{2} \bigg(\log e_i - \log \sigma + \int \mathcal{N}(\epsilon_i; 0, \I) \epsilon_{i}^T \epsilon_{i} d \epsilon_i - D \log 2 \pi \bigg) \\
&\approx \sum_{i=1}^2 \frac{e_i}{2} \big( -\log \sigma - D (1+\log 2 \pi) \big) - \frac{1}{2}H(e)
\end{align}

\begin{align}
\int q_\theta(\omega) \log p(\omega) d\omega &= \sum_{i=1}^2 e_i \int \mathcal{N}(\omega; \theta_i, \sigma^2_i\mathbf{I}) \log \mathcal{N}(\omega; 0, \mathbf{I}) d\omega \\
&= -\frac{1}{2}\sum_{i=1}^2 e_i \big( \theta_i^T \theta_i + D\sigma \big)
\end{align}
Then we can approximate
\begin{align}
\mathrm{KL}(q_\theta(\omega) || p(\omega)) &\approx \sum_{i=1}^2 \frac{e_i}{2} \big(\theta_i^T \theta_i +D\sigma - \log \sigma - D (1+\log 2 \pi) \big) - \frac{1}{2}H(e)
\end{align}


